A Survey of Evaluation Metrics Used for NLG Systems

The success of Deep Learning has created a surge in interest in a wide a range of Natural Language Generation (NLG) tasks. Deep Learning has not only pushed the state of the art in several existing NLG tasks but has also facilitated researchers to explore various newer NLG tasks such as image captioning. Such rapid progress in NLG has necessitated the development of accurate automatic evaluation metrics that would allow us to track the progress in the field of NLG. However, unlike classification tasks, automatically evaluating NLG systems in itself is a huge challenge. Several works have shown that early heuristic-based metrics such as BLEU, ROUGE are inadequate for capturing the nuances in the different NLG tasks. The expanding number of NLG models and the shortcomings of the current metrics has led to a rapid surge in the number of evaluation metrics proposed since 2014. Moreover, various evaluation metrics have shifted from using pre-determined heuristic-based formulae to trained transformer models. This rapid change in a relatively short time has led to the need for a survey of the existing NLG metrics to help existing and new researchers to quickly come up to speed with the developments that have happened in NLG evaluation in the last few years. Through this survey, we first wish to highlight the challenges and difficulties in automatically evaluating NLG systems. Then, we provide a coherent taxonomy of the evaluation metrics to organize the existing metrics and to better understand the developments in the field. We also describe the different metrics in detail and highlight their key contributions. Later, we discuss the main shortcomings identified in the existing metrics and describe the methodology used to evaluate evaluation metrics. Finally, we discuss our suggestions and recommendations on the next steps forward to improve the automatic evaluation metrics.

==> MT_metrics_WMT19.tex <==
 \begin{table}[h]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c}
         Translation & de-en & fi-en & gu-en & kk-en & lt-en & ru-en & zh-en \\
         \hline
         %Segment-level & Yisi1 \cite{DBLP:conf/wmt/Lo19_yisi} & Yisi, ESIM &
         to English & Yisi1 \cite{DBLP:conf/wmt/Lo19_yisi} & Meteor++ 2.0 \cite{DBLP:conf/wmt/GuoH19_meteorpp2}, BEER \cite{DBLP:conf/wmt/StanojevicS15_beer_metric} & Yisi0 \cite{DBLP:conf/wmt/Lo19_yisi} & WMDO \cite{chow-etal-2019-WMDO} & ESIM \cite{DBLP:conf/acl/ChenZLWJI17_ESIM_for_inference,DBLP:conf/acl/MathurBC19_BERTr_contextualized_embeddings_translation} & Yisi1, BERTr \cite{DBLP:conf/acl/MathurBC19_BERTr_contextualized_embeddings_translation} & ESIM \\
         %from Eng & Yisi1, ESIM & BEER, Yisi0, EED \cite{_eed} & characTER \cite{DBLP:conf/wmt/WangPRN16_characTER}, Yisi1 & Yisi1, ESIM & TER \cite{Snover06astudy_ter} & Yisi1
         from Eng & Yisi1, ESIM & BEER, Yisi0, EED \cite{stanchev-etal-2019-eed} & characTER \cite{DBLP:conf/wmt/WangPRN16_characTER} & Yisi1, ESIM &TER,NIST\cite{10.5555/1289189.1289273_nist} & TER \cite{Snover06astudy_ter} & Yisi1
    \end{tabular}
    \caption{Metrics achieving the maximum pearson correlation for each language pair in WMT19 dataset. Note: These are system level correlations. Maximum segment-level correlations are quite underwhelming (<0.4) Reference: \citet{DBLP:conf/wmt/MaWBG19} }
    \label{tab:trans_best_corr}
\end{table}

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> datasets.tex <==

\section{Datasets}
In this section, we briefly describe the commonly used datasets which provide human scores for training/evaluating NLG metrics. %\Ana{The datasets below are only the ones which provide large-scale human judgements. I'm thinking we could have this section and Challenges and Datasets and discuss WMT, WebNLG challenge and DUC instead? Perhaps in a later iteration of the paper?}\\

\noindent \textbf{WMT Shared Metric Task:} The WMT shared Metric task is an annual task on automatic evaluation metrics for machine translation since 2008. The task involves automatically evaluating translations produced in the WMT shared translation task using the human reference translations. The training dataset for the task also includes human ratings for the pairs of sentences. For the years 2017, 2018, and 2019, the training sets contain 5,360, 9,492, and 147,691 records. The evaluation metrics are assessed based on correlations with human judgements at both the system and sentence level using either Pearson correlation or the custom Kendall's $\tau$ as described in the previous section. \\

\noindent \textbf{WebNLG:} The WebNLG challenge consist of converting data into natural language text. The data is a set of triples extracted from DBpedia and the text is a verbalisation of these triples. The organizers released the human judgements for 4,677 sentence pairs that span 9 systems. Human judgements are made based on 3 criteria \textit{viz, } fluency, semantics, and grammar. \\

\noindent \textbf{Human Judgements from Persona Chat:}  \cite{DBLP:conf/naacl/SeeRKW19} conducted a large-scale human evaluation study to measure the effect of various controllable parameters in neural text generation models on the PersonaChat task \cite{personachat}. The study involved human-system conversations from 28 model configurations and also had human-human conversations for comparison. Human annotators interacted with a system/another human and rated the conversational quality on a scale of 1-3 based on 8 criteria \textit{viz.} avoiding repetition, interestingness, making sense, fluency, listening, inquisitiveness, humanness and engagingness. 

% WebNLG, ParaNMT, WMT

==> que.tex <==
\section{Criticisms of existing automated metrics}
Within 2 years from when BLEU and NIST were proposed, \citet{DBLP:conf/lrec/ZhangVW04_bleu_nist_quant_imprvment} made an analysis of the flaws in these metrics including the difficulty in interpreting the comparisons of different MT systems using these scores or quantifying any improvements in the tasks. \citet{article_early_mt_eval_comp} compare the various automatic metrics and human-based metrics for translation and have %some interesting points regarding
demonstrated the influence of references in automatic metrics as well as the subjectiveness of the human judges in human-based evaluations.\\
 %(Additionally, check if sentBLEU also a standardization?) %ways to compare
% A structured review of the validity of bleu.
%\subsection{Shortcomings of existing metrics}
%Should we have this section split into sections on criticisms after each subset of metrics discussed?\\
%write about studies showing poor correlations, etc.\\
\citet{10.1007/978-3-540-30586-6_38_critique1} report negative correlation of BLEU, NIST, SSA (Simple String Accuracy) \cite{DBLP:conf/inlg/BangaloreRW00_ssa}, Melamed's F-measure (i.e., GTM \cite{article_general_text_matcher_gtm}), and LSA (Latent Semantic Analysis) \cite{DBLP:journals/jasis/DeerwesterDLFH90_LSA} with human judgements on fluency, with barely decent correlations on adequacy scores. They suggest evaluating adequacy, fluency and readability separately.  %(amidst other directions such as tree-based methods)
\citet{belz-reiter-2006-comparing_auto_human_nlg_eval} stress on the influence of corpus-quality on the correlations between human and automatic evaluation schemes, observing that large number of good quality references lead to better correlations.\\
In fact, one of the major recurring criticism of the automatic metrics is regarding their poor correlation human judgements. This has been shown for various NLG tasks with various datasets as summarized in Table \ref{tab:critic_corrs}.\\
\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c}
         Work & Metrics & Datasets \\ \hline
         \cite{DBLP:conf/emnlp/NovikovaDCR17} & BLEU, TER, ROUGE, NIST, LEPOR, METEOR, CIDEr & BAGEL \cite{mairesse-etal-2010_bagel_dataset}, SF-HOTEL, SF-RESTAURANT \cite{wen-etal-2015_sfhotel_rest_dataset}\\
         \cite{DBLP:conf/acl/ElliottK14} & Smoothed-BLEU \cite{DBLP:conf/acl/ClarkDLS11_smoothedbleu}, TER, ROUGE-SU4, Meteor  & Flickr8K\cite{DBLP:journals/jair/HodoshYH13_flickr8k}, E\& K\cite{DBLP:conf/emnlp/ElliottK13_EKdataset}\\
         \cite{kryscinski-etal-2019-neural_summ_critic} & ROUGE-1,2,L & CNN/DailyMail\\
         \cite{DBLP:journals/csl/DusekNR20_e2enlg} & BLEU, NIST, METEOR, ROUGE-L, CIDEr & E2E NLG dataset\\
         \cite{DBLP:conf/emnlp/NemaK18_qbleu} & BLEU, ROUGE-L, NIST, METEOR& SQuAD, WikiMovies, VQA\\
         \cite{DBLP:conf/acl/DhingraFPCDC19_parent} & ROUGE, CIDEr, METEOR, BLEU, CS & WikiBio\\
         \cite{DBLP:journals/corr/abs-1807-02202_chaganty} & BLEU, ROUGE, METEOR, VecSim & MS MARCO, CNN/DailyMail  \\
         \cite{DBLP:conf/emnlp/LiuLSNCP16HowNot} & BLEU, ROUGE, METEOR, Greedy matching, vector extrema/avg & Twitter, Ubuntu\\
         \cite{DBLP:conf/acl-mrqa/ChenSSG19} & BLEU, ROUGE, SMS, BERTScore & NarrativeQA, SemEval, ROPES\\
    \end{tabular}
    \caption{Works showing poor correlation of various metrics with human judgements on various datasets}
    \label{tab:critic_corrs}
\end{table}\\
\citet{DBLP:conf/wmt/MaWBG19} show correlations are not reliable if all the translation systems to be ranked are all good systems. %and similar.
Building upon this, \citet{DBLP:journals/corr/abs-2006-06264_tangled_up_in_bleu} show that this difficulty in ranking the good systems is applicable in general to ranking any set of systems that are of similar capability. They also observe that one has to eliminate outliers (and follow other relevant bias and noise eliminating strategies) to get more reliable and robust correlations to compare the various metrics.
\cite{kryscinski-etal-2019-neural_summ_critic} criticize both the human evaluations as well as automatic metrics for abstractive summarization since neither of those check for factual inconsistencies in the summaries. They also call attention to potential problems in the datasets including Layout bias in news datasets and noise in any web-scraped datasets.\\
\citet{DBLP:journals/nle/GrahamBMZ17_crowd_alone} examine whether the assessment of the MT evaluation metrics is robust and if monolingual evaluators can be relied upon for human evaluations as opposed to experts or biligual evaluators. %address the question "Can machine translation systems be evaluated by the crowd alone". (Do they also give us DA, i.e., Direct Assessment?)\\
\cite{DBLP:journals/csl/DusekNR20_e2enlg} note the varied ranking outcomes when using automatic versus human evaluations. They find that with most automatic metrics, the fluency of the language can be reliably determined and seq2seq models perform well. However in terms of adequacy and correctness, on which the automatic metrics do not agree with human evaluations, seq2seq models perform worse than rule-based models, but they still manage to procure high scores on the automatic metrics. \\% between that seq2seq models 
\cite{DBLP:journals/corr/abs-1807-02202_chaganty} also report the effects of having good quality (low variance) human judgements as well as improved correlations of the automatic metrics to optimize evaluation costs. They compare various settings for human evaluation, including Likert scale prompt for scoring overall quality, or quantifying the post-editing costs. They also ask the annotators to highlight the regions of text that support their decision in question answering task. They also report their finding that learned metrics are difficult to generalize to evaluate different systems. \\  %Chaganty and Novikova additionally find that correlations vary across systems
%"The price of debiasing automatic metrics in natural language evaluation" by \citet{DBLP:journals/corr/abs-1807-02202_chaganty}\\
Under the dialogue setting, \cite{DBLP:conf/emnlp/NovikovaDCR17} find that utterances with low human scores on informativeness and naturalness correlate significantly better with the automatic scores than utterances with good or average human scores. They also assess the quality of the data and examine its characteristics such as the length of the references, words,  characters, or syllables per sentence, etc in the dataset and find that these measures influence the correlations. Their results re-confirm the findings that automatic metrics are reliable at the system-level \cite{DBLP:journals/coling/ReiterB09} and less so at the sentence-level \cite{10.1007/978-3-540-30586-6_38_critique1}.\\
%"Why we need new evaluation metrics for NLG" by \citet{DBLP:conf/emnlp/NovikovaDCR17}\\
"How not to Evaluate..." by \citet{DBLP:conf/emnlp/LiuLSNCP16HowNot}. This is specifically related to dialogues.\\
Similarly, specific ones to NMT follow here\\
"Re-evaluating the role of BLEU in machine translation research" by \citet{callison-burch-etal-2006-evaluating_bleu_in_mt} shows that rule-based systems receive low BLEU scores. (Why?) \\
"A structured review of the validity
of BLEU" by \citet{DBLP:journals/coling/Reiter18_validity_of_bleu} analyses how BLEU correlations have changed over the years.\\
"Some Issues in Automatic Evaluation of English-Hindi MT: More Blues for BLEU" by \citet{Ananthakrishnan2006SomeII_more_blues} \\
" Re-evaluating  automatic metrics   for   image   captioning" by \citet{DBLP:conf/eacl/KilickayaEIE17_reeval_IC_metrics}.\\
"Challenges in Data-to-Document Generation" by \citet{DBLP:conf/emnlp/WisemanSR17} on Data-to-Text tasks. (Also refer \citet{DBLP:journals/corr/abs-1910-08684_wikibio_confidence} for other identifications to go in this section and/or others.)\\
In comparing the existing metrics and deciding the significance of "improvements":\\


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Criticism studies on the existing automatic metrics}
Automatic metrics have been critically examined to understand their shortcomings or loopholes.
 %(Additionally, check if sentBLEU also a standardization?) %ways to compare
% A structured review of the validity of bleu.
%\subsection{Shortcomings of existing metrics}
%Should we have this section split into sections on criticisms after each subset of metrics discussed?\\
%write about studies showing poor correlations, etc.\\
%Many metrics 
%BLEU being old, popular -> under scrutiny
% -poor correlation
% -interpretability
% -divergence and language
% -adaptability to the task and solving the task
\subsection{Poor Correlations}
\citet{10.1007/978-3-540-30586-6_38_critique1} report negative correlation of BLEU, NIST, SSA (Simple String Accuracy) \cite{DBLP:conf/inlg/BangaloreRW00_ssa}, Melamed's F-measure (i.e., GTM \cite{article_general_text_matcher_gtm}), and LSA (Latent Semantic Analysis) \cite{DBLP:journals/jasis/DeerwesterDLFH90_LSA} with human judgements on fluency, with barely decent correlations on adequacy scores. They suggest evaluating adequacy, fluency and readability separately.  %(amidst other directions such as tree-based methods)
In fact, one of the major recurring criticism of the automatic metrics is regarding their poor correlation human judgements. This has been shown for various NLG tasks with various datasets as summarized in Table \ref{tab:critic_corrs}.\\
\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c}
         Work & Metrics & Datasets \\ \hline
         \cite{DBLP:conf/emnlp/NovikovaDCR17} & BLEU, TER, ROUGE, NIST, LEPOR, METEOR, CIDEr & BAGEL \cite{mairesse-etal-2010_bagel_dataset}, SF-HOTEL, SF-RESTAURANT \cite{wen-etal-2015_sfhotel_rest_dataset}\\
         \cite{DBLP:conf/acl/ElliottK14} & Smoothed-BLEU \cite{DBLP:conf/acl/ClarkDLS11_smoothedbleu}, TER, ROUGE-SU4, Meteor  & Flickr8K\cite{DBLP:journals/jair/HodoshYH13_flickr8k}, E\& K\cite{DBLP:conf/emnlp/ElliottK13_EKdataset}\\
         \cite{kryscinski-etal-2019-neural_summ_critic} & ROUGE-1,2,L & CNN/DailyMail\\
         \cite{DBLP:journals/csl/DusekNR20_e2enlg} & BLEU, NIST, METEOR, ROUGE-L, CIDEr & E2E NLG dataset\\
         \cite{DBLP:conf/emnlp/NemaK18_qbleu} & BLEU, ROUGE-L, NIST, METEOR& SQuAD, WikiMovies, VQA\\
         \cite{DBLP:conf/acl/DhingraFPCDC19_parent} & ROUGE, CIDEr, METEOR, BLEU, CS & WikiBio\\
         \cite{DBLP:journals/corr/abs-1807-02202_chaganty} & BLEU, ROUGE, METEOR, VecSim & MS MARCO, CNN/DailyMail  \\
         \cite{DBLP:conf/emnlp/LiuLSNCP16HowNot} & BLEU, ROUGE, METEOR, Greedy matching, vector extrema/avg & Twitter, Ubuntu\\
         \cite{DBLP:conf/acl-mrqa/ChenSSG19} & BLEU, ROUGE, SMS, BERTScore & NarrativeQA, SemEval, ROPES\\
    \end{tabular}
    \caption{Works showing poor correlation of various metrics with human judgements on various datasets}
    \label{tab:critic_corrs}
\end{table}\\
\citet{DBLP:conf/wmt/MaWBG19} show correlations are not reliable if all the translation systems to be ranked are all good systems. %and similar.
Building upon this, \citet{DBLP:journals/corr/abs-2006-06264_tangled_up_in_bleu} show that this difficulty in ranking the good systems is applicable in general to ranking any set of systems that are of similar capability. %They also observe that one has to eliminate outliers (and follow other relevant bias and noise eliminating strategies) to get more reliable and robust correlations to compare the various metrics. 
In contrast, at the sentence level, \citet{DBLP:journals/coling/FomichevaS19_correlation_1} find that metrics are better at distinguishing between high-quality translations compared to low-quality translations.
%Similarly, 
However, under the dialogue setting, \cite{DBLP:conf/emnlp/NovikovaDCR17} find that utterances with low human scores on informativeness and naturalness correlate significantly better with the automatic scores than utterances with good or average human scores. 
Overall, many studies  \cite{DBLP:journals/coling/Reiter18_validity_of_bleu,DBLP:conf/emnlp/NovikovaDCR17,DBLP:conf/acl/DhingraFPCDC19_parent} re-confirm the findings that automatic metrics are reliable at the system-level \cite{DBLP:journals/coling/ReiterB09} and less so at the sentence-level \cite{10.1007/978-3-540-30586-6_38_critique1}. %results
%\\  %Chaganty and Novikova additionally find that correlations vary across systems
%"The price of debiasing automatic metrics in natural language evaluation" by \citet{DBLP:journals/corr/abs-1807-02202_chaganty}\\

\subsection{Task-specific criticisms/ shortcomings}
Most of the NLG tasks still have automatic metrics poorly correlated with the human judgements. We discuss the other task-specific problems which could also be the reasons behind poor correlations.
%There are however, other problems which might or might not be reasons for the poor correlations, which we discuss here.
\citet{kryscinski-etal-2019-neural_summ_critic} criticize both the human evaluations as well as automatic metrics for abstractive summarization since neither of those check for factual inconsistencies in the summaries. Similarly \citet{DBLP:conf/emnlp/WisemanSR17} discuss the lack of a reliable measurement of faithfulness in the context of Data-to-Text Generation. Further, \citet{DBLP:conf/acl/DhingraFPCDC19_parent} show that references provided for this task might contain additional information which is not present in the semi-structured data (as in WikiBio), and allude automatic metrics to be more reliant upon the context. % which cannot be expected to be produced by the systems. % and that such divergence would lead to improper judgements on the hypothesis.
\citet{Ananthakrishnan2006SomeII_more_blues} particularly look at the Hindi-English translation task and list the various issues and divergence in the language-pair that are not effectively captured by BLEU. These include lexical, categorical, pleonastic, and stylistic divergence, Word-sense Disambiguation, identification of transliteration, and non-perfect or indicative translations.
\citet{DBLP:conf/emnlp/LiuLSNCP16HowNot} find that none of the untrained metrics are able to capture the diversity of valid responses and criticize the adoption of metrics proposed for other NLG tasks to evaluate dialogues. They also point out the difference in the usage of some of these metrics, which originally take in multiple references, on dialogue datasets which often have a single reference. Another noteworthy point is that the untrained automatic metrics only consider the reference without taking into account the context, which is required to determine the validity of a response. 
%" Re-evaluating  automatic metrics for image  captioning" by \citet{DBLP:conf/eacl/KilickayaEIE17_wmd_ic}.
%"Challenges in Data-to-Document Generation" by \citet{DBLP:conf/emnlp/WisemanSR17} on Data-to-Text tasks. (Also refer \citet{DBLP:journals/corr/abs-1910-08684_wikibio_confidence} for other identifications to go in this section and/or others.)\\
%"How not to Evaluate..." by \citet{DBLP:conf/emnlp/LiuLSNCP16HowNot}. This is specifically related to dialogues.\\
%Similarly, specific ones to NMT follow here\\
\subsection{Metric-specific criticisms}
The wide-spread use of BLEU as an evaluation metric for many NLG tasks has led to it being under constant scrutiny, questioning its deployment in various tasks. Within 2 years from when BLEU and NIST were proposed, \citet{DBLP:conf/lrec/ZhangVW04_bleu_nist_quant_imprvment} made an analysis of the flaws in these metrics including the difficulty in interpreting the scores, and thereby problems in comparing different MT systems using these scores, and quantifying any improvements in the tasks. \citet{callison-burch-etal-2006-evaluating_bleu_in_mt} demonstrate that BLEU score improvement is neither sufficient nor necessary to indicate progress in translation task by showing its susceptibility to equally score all the different permutations of the phrases or n-grams of the hypothesis. These permutations can also be generated from the n-grams of the references. In other words, BLEU admits many spurious variants and penalizes correct translations if they substantially differ from the vocabulary of the references. The authors also support the finding in \cite{coughlin2003correlating} that BLEU is favorably biased towards n-gram-based translation systems over rule-based systems. %and suggest using BLEU to check for broad incremental changes in systems that employ same techniques (such as phrase-based translation
They suggest that these drawbacks also hold for other metrics such as METEOR, GTM, etc.
%"Re-evaluating the role of BLEU in machine translation research" by \citet{callison-burch-etal-2006-evaluating_bleu_in_mt} shows that rule-based systems receive low BLEU scores. (Why?) 
%\citet{Ananthakrishnan2006SomeII_more_blues} particularly look at the Hindi-English translation task and list the various issues and divergence in the language-pair that are not effectively captured by BLEU. These include lexical, categorical, pleonastic, and stylistic divergence, Word-sense Disambiguation, identification of transliteration, and non-perfect or indicative translations. %partial % and issues in the two translations
Finally \citet{DBLP:journals/coling/Reiter18_validity_of_bleu} analyses the varying BLEU correlations in various reports over 15 years and recommend that BLEU only be used as a coarse system-level metric for MT evaluation, and not for other NLG tasks. %summarize the results  %coarse indicator
Among the trained metrics, \cite{DBLP:conf/aaai/SaiGKS19Reeval} find that ADEM always scores the dialogue responses, whether relevant or not, in a narrow range around the median and observe that all the response encodings by ADEM are also banded together in the vector space with high conicity. %They also show that ADEM is susceptible to various synthetic and white-box attacks. 
%"A structured review of the validity of BLEU" by \citet{DBLP:journals/coling/Reiter18_validity_of_bleu} analyses how BLEU correlations have changed over the years.
%"Some Issues in Automatic Evaluation of English-Hindi MT: More Blues for BLEU" by \citet{Ananthakrishnan2006SomeII_more_blues} \\
%%In comparing the existing metrics and deciding the significance of "improvements":\\

==> reqments.tex <==
\subsection{Mandatory requirements}
\textbf{Fluency:} Fluency or grammatical correctness is necessary for any NLG system. The syntax varies for different languages.\\
\textbf{Sensibility:} The hypothesis should be logically sound within itself, being meaningful and not containing any self-contradicting information.\\ %Integrity: The hypothesis should be logically sound within itself, without containing any contradicting statements
\textbf{Unambiguity:} The hypothesis generated should be as clear as possible.\\
\textbf{Coherence }(w.r.t context): The message contained in the generated text should be consistent with the information present in the context. \\
\textbf{Common sense:} Adhering to universal facts and common sense information in the text is a desirable additional feature.\\
\textbf{Adequacy and Task fulfillment:}
%Inspite of the above qualities, 
The generated text also needs to address the task requirements, along with the above factors. We define this as `task fulfillment'. Since the definition of adequacy differs for each task, we discuss them separately for each task, coupling it with task fulfillment:
\begin{itemize}
    \item \textbf{Machine Translation} task requires complete information in the source language text to be retained in the target language translation.
    \item \textbf{Automatic Summarization} task requires correct identification of the key idea or the few main points which are to be summarized, maintaining coherence with the original text. Here adequacy is with respect to the key points and not the "completeness" w.r.t the whole text.
    \item \textbf{Question Answering} task where the answers are to be generated instead of selected from the text or out of given options, needs to be both sound and complete w.r.t the question as well as any background information (passage, image, knowledge base, common sense and universal facts, etc).
    \item \textbf{Question Generation} needs the question to be related to the base material it is based upon (i.e., passage/image, etc) and additionally be answerable with the given information..
    \item \textbf{Data to Text generation} needs facts to be preserved, while adequately verbalizing the information present in tables or other data forms.
    \item \textbf{Image Captioning} task expects captions to be relevant to the image, without stating anything contradicting the image. The caption need not describe everything in the image, as long as it focuses on the significant details or the theme of the image.
    \item \textbf{Automated Dialogue} agents need to ``listen" to the other speaker, thereby adequately respond. The utterances also have to be coherent/consistent with the agent's own previous utterances, as well as the other speaker's utterances. %We term this requirement `consistency', where most of the 
\end{itemize}
From the above elaboration, it is evident that certain mandatory requirements are applicable only to a subset of the tasks, which we discuss below.\\%such as answerability. %We mention some of the factors which are required 
\textbf{Answerability:} For any question generation task, the question might not be answerable due to lack of completeness or sensibility, or even because the information required to answer the question might not be in the context. While the last case is acceptable since such questions can be answered stating the insufficiency of information, answerability is desired and important for generating meaningful questions overall.\\
\textbf{Dialogue flow:} Conversations have an interlinking quality across utterances, and maintain coherence of information throughout. Additionally, (open-domain) dialogue agents need to display:
\begin{itemize}
    \item Emotional consistency
    \item Personality consistency
\end{itemize}
\subsection{Additional requirements}
\textbf{Creativity:} A machine that exhibits its creativity could be desired for certain specific adaptations of the NLG tasks. Creativity can be enhanced through connecting additional components or abstraction, which would make this criteria more applicable to tasks with a certain degree of freedom for generating text, such as image captioning, summarization, question generation, and dialogues.\\
\textbf{Brief vs Detailed:} Depending on the task requirements, either brief or detailed generations might be preferred.\\
%Optimal: (brief or elaborate) - depending on the requirement
%Answerability
\textbf{Engagingness: } This is again specific to dialogues. Given the diversity of possible ways a conversation can proceed, engagingness becomes a significant criteria for chatbot evaluation.\\
%Emotional consistency
%Personality consistency
\textbf{Style: } The generated text might need to be more formal or colloquial, depending on the end application. Alternatively, we might want the text in the style of a particular person, era, etc.\\


\section{Human Evaluation of NLG systems}
%Wishlist for NLG evaluation metrics
%An NLG evaluation metric has a multitude of conditions/parameters to check and analyze for providing an appropriate score on a generated hypothesis. The bare minimum checks are for good grammar (fluency) and the correctness of the outcome with respect to the expected requirements of the specific task. There could be additional parameters to judge upon for each NLG task, to understand the progress in the field and compare the various models or solutions. For example, in Automated Dialogues, a system that is more engaging would be preferred for application in open-domain chitchat, when compared against other systems of same levels of fluency and correctness. Engaging-ness is an additional prize-winning factor for dialog systems, but is irrelevant to a translation system. We hence discuss the various parameters that influence evaluation, also specifying the tasks that take them into consideration, if applicable. We classify the evaluation parameters into mandatory (bare-minimum) requirements and additional requirements. The idea is that the NLG models need to satisfy all the mandatory requirements, and the additional factors can then determine their competitiveness and application.
Human evaluation would be ideal to evaluate any generated hypothesis or even NLG systems as a whole. However, human evaluations are difficult to obtain on a large-scale and are expensive and time consuming. However, human evaluations are usually reported on a sample of the data to show advancement in an NLG model or to compare the correlation with automatic metrics. In this section we provide a summary of human evaluations, particularly the procedures adopted for setting up such evaluations and the parameters evaluated for various NLG tasks.\\ 
%An NLG evaluation metric has a multitude of conditions/parameters to check and analyze for providing an appropriate score on a generated hypothesis. The bare minimum checks are for good grammar (or fluency) and the correctness of the outcome with respect to the expected requirements of the specific task. There could be additional parameters to judge upon for each NLG task, to understand the progress in the field and compare the various models or solutions. For example, in Automated Dialogues, a system that is more engaging would be preferred for application in open-domain chitchat, when compared against other systems of same levels of fluency and correctness. Engaging-ness is an additional prize-winning factor for dialog systems, but is irrelevant to a translation system. We hence discuss the various parameters that matter for evaluation separately for each NLG task, further dividing them into mandatory (bare-minimum) factors and additional factors. The idea is that the NLG models need to %first be able to 
%satisfy all the mandatory requirements, and the additional factors can then determine their competitiveness and application.
%Now formally list down and define the union of all human measures which were carefully referred to earlier: fluency, adequacy, coherency, answerability etc. Draw a task $\times$ measure matrix. This matrix will have checkmarks in the appropriate cells. For example, the cell \{NMT, answerability\} will not have a checkmark.\\
% \begin{table}[t]
%     \centering
%     \begin{tabular}{c|c|c|c|c|c|c}
%          NLG task & Fluency & Adequacy & Coherence & Answerability & Creativity & Engagingness \\
%          \hline
%          MT & \checkmark & \checkmark & \checkmark & & &\\
%          AS & \checkmark & (\checkmark) & \checkmark & & &\\
%          QA & \checkmark & \checkmark &  \checkmark & & & \\
%          QG & \checkmark & & \checkmark & \checkmark & \checkmark &\\
         
%          D2T & \checkmark & \checkmark &  \checkmark & & &\\
%          AD & \checkmark & \checkmark &  \checkmark & & \checkmark & \checkmark\\
%          IC & \checkmark & \checkmark &  \checkmark & & \checkmark &\\
%     \end{tabular}
%     \caption{Wishlist for various NLG tasks. (MT: Machine Translation, AS: Automatic Summarization, QA: Question Answering, QG: Question Generation, D2T: Data to text, AD: Automated Dialogues, IC: Image captioning}
%     \label{tab:wishlist}
% \end{table}
%%TODO: Change the table to instead have entries on which metric has been used for which task
%\subsection{Mandatory requirements}
%\textbf{Rating the task:}
\subsection{Evaluating Fulfillment of Task Requirements}
Most human evaluations check for task fulfillment as a whole. That is, humans are asked to rate or compare the generated sentences (and the generating systems) to indicate how satisfactorily it meets the task requirements overall  \cite{DBLP:conf/acl/LoweNSABP17ADEM,DBLP:conf/wmt/MaBG18,DBLP:conf/wmt/MaWBG19,ghazarian19}.\\ %Ghazarian -> not appropriate to very appropriate. ADEM- overall quality of the response. RUBER -> human satisfaction of a reply.
\textbf{Machine Translation} task requires complete information in the source language text to be retained in the target language, without the introduction of any additional elements/aspects to the text.\\
\textbf{Automatic Summarization} task requires correct identification of the key idea or the few main points which are to be summarized, and provide a summary maintaining coherence with the original text.\\
\textbf{Question Answering} task where the answers are to be generated (instead of selected from the text or out of given options) need to effectively address the question and maintain coherence with the question as well as any background information (passage, knowledge base, common sense and universal facts, etc).\\
\textbf{Question Generation} needs the question to be related to the base material it is based upon (i.e., passage/image, etc) and additionally be answerable with the given information.\\
\textbf{Data to Text generation:} It is important for the text to preserve the facts as well as be adequate in verbalizing the information present in the data.\\
\textbf{Automated Dialogue} agents need to "listen" to the other speaker, thereby adequately respond. That is, the generated response should be coherent with the agent's own previous utterances, as well as the other speaker's utterances.\\
\textbf{Image Captioning:} The caption should be relevant to the image and adequately explain the image. Although it need not describe everything in the image and can mostly focus on the significant details, the caption cannot contradict the image.
\subsubsection{Human-likeness:} Often the human evaluation for these various tasks is summarized into one entity measuring how human-like the generated sentence is.
\subsection{Evaluating Contributing Factors Individually}
Evaluations can also be performed at a more fine-grained level where different factors are individually scored. % as done by \citet{DBLP:journals/corr/abs-2005-00583_maude,DBLP:conf/naacl/SeeRKW19}.\\
The factorization is task-specific and the level of granularity varies. \cite{DBLP:conf/naacl/SeeRKW19} and \cite{DBLP:journals/corr/abs-2005-00583_maude} evaluate conversation systems for for Engagingness, Interestingness, Inquisitiveness, Listening, Avoiding Repetition, Fluency, Making Sense, Ease of Persona retrieval, and Humanness. \cite{DBLP:conf/emnlp/NemaK18_qbleu} evaluate the task of Question Generation using the parameter of `answerability'.
\subsection{Human Evaluation Setup}
%The human evaluators could be experts or even new to the task. 
The sentences to be evaluated are presented to human annotators who might be asked to score the hypothesis individually or compare it against another.\\
Likert scale: (getting a score on a scale, say 1-5).
Also check \citet{DBLP:conf/emnlp/NovikovaDCR17} for comments on human scale varying from metric scale, and that extremes are easily classified than middle scores. "While discrete, ordinal scales are the dominant method, a continuous scale - for example, one involving a visually presented slider (Gatt \& Belz, 2010; Belz \& Kow, 2011) - might give subjects the possibility of giving more nuanced judgements." \\
Acute-EVAL by \citet{DBLP:journals/corr/abs-1909-03087_acute_eval} : Humans compare models and pass pairwise judgement based on preference. Pitched in the context of dialogues.\\
%\textbf{Fluency:} Checking for grammatical correctness\\
%\textbf{Sensibility:} Indicating whether the hypothesis is meaningful \\
% \textbf{Fluen%cy:} Fluency or grammatical correctness is necessary for any NLG system. The syntax varies for different languages.\\
% \textbf{Sensibility:} The hypothesis should be logically sound within itself, being meaningful and not containing any self-contradicting information.\\ %Integrity: The hypothesis should be logically sound within itself, without containing any contradicting statements
% \textbf{Unambiguity:} The hypothesis generated should be as clear as possible.\\
% \textbf{Coherence }(w.r.t context): The message contained in the generated text should be consistent with the information present in the context. \\
% \textbf{Common sense:} Adhering to universal facts and common sense information in the text is a desirable additional feature.\\
% \textbf{Adequacy and Task fulfillment:}
% %Inspite of the above qualities, 
% The generated text also needs to address the task requirements, along with the above factors. We define this as `task fulfillment'. Since the definition of adequacy differs for each task, we discuss them separately for each task, coupling it with task fulfillment:
% \begin{itemize}
%     \item \textbf{Machine Translation} task requires complete information in the source language text to be retained in the target language translation.
%     \item \textbf{Automatic Summarization} task requires correct identification of the key idea or the few main points which are to be summarized, maintaining coherence with the original text. Here adequacy is with respect to the key points and not the "completeness" w.r.t the whole text.
%     \item \textbf{Question Answering} task where the answers are to be generated instead of selected from the text or out of given options, needs to be both sound and complete w.r.t the question as well as any background information (passage, image, knowledge base, common sense and universal facts, etc).
%     \item \textbf{Question Generation} needs the question to be related to the base material it is based upon (i.e., passage/image, etc) and additionally be answerable with the given information..
%     \item \textbf{Data to Text generation} needs facts to be preserved, while adequately verbalizing the information present in tables or other data forms.
%     \item \textbf{Image Captioning} task expects captions to be relevant to the image, without stating anything contradicting the image. The caption need not describe everything in the image, as long as it focuses on the significant details or the theme of the image.
%     \item \textbf{Automated Dialogue} agents need to ``listen" to the other speaker, thereby adequately respond. The utterances also have to be coherent/consistent with the agent's own previous utterances, as well as the other speaker's utterances. %We term this requirement `consistency', where most of the 
% \end{itemize}
% From the above elaboration, it is evident that certain mandatory requirements are applicable only to a subset of the tasks, which we discuss below.\\%such as answerability. %We mention some of the factors which are required 
% \textbf{Answerability:} For any question generation task, the question might not be answerable due to lack of completeness or sensibility, or even because the information required to answer the question might not be in the context. While the last case is acceptable since such questions can be answered stating the insufficiency of information, answerability is desired and important for generating meaningful questions overall.\\
% \textbf{Dialogue flow:} Conversations have an interlinking quality across utterances, and maintain coherence of information throughout. Additionally, (open-domain) dialogue agents need to display:
% \begin{itemize}
%     \item Emotional consistency
%     \item Personality consistency
% \end{itemize}
% \subsection{Additional requirements}
% \textbf{Creativity:} A machine that exhibits its creativity could be desired for certain specific adaptations of the NLG tasks. Creativity can be enhanced through connecting additional components or abstraction, which would make this criteria more applicable to tasks with a certain degree of freedom for generating text, such as image captioning, summarization, question generation, and dialogues.\\
% \textbf{Brief vs Detailed:} Depending on the task requirements, either brief or detailed generations might be preferred.\\
% %Optimal: (brief or elaborate) - depending on the requirement
% %Answerability
% \textbf{Engagingness: } This is again specific to dialogues. Given the diversity of possible ways a conversation can proceed, engagingness becomes a significant criteria for chatbot evaluation.\\
% %Emotional consistency
% %Personality consistency
% \textbf{Style: } The generated text might need to be more formal or colloquial, depending on the end application. Alternatively, we might want the text in the style of a particular person, era, etc.\\

% \textbf{General NLG requirements:} Good grammar (fluency) and logic/soundness (encompassing both the integrity of the standalone generated text, as well as its faithfulness to a base material - image, passage, etc). The thresholds for some of the metrics vary across tasks. For eg: in MT, we want all the information to be translated, but for image captioning, skipping some details from the image would be acceptable while generating the caption. So, the thresholds for adequacy can change.\\
% \textbf{Machine Translation} task requires complete information in the source language text to be retained in the target language, without the introduction of any additional elements/aspects to the text.\\
% \textbf{Automatic Summarization} task requires correct identification of the key idea or the few main points which are to be summarized, maintaining coherence with the original text. Here adequacy is with respect to the key points and not the "completeness" w.r.t the whole text.\\
% \textbf{Question Answering} task where the answers are to be generated instead of selected from the text or out of given options need to be both sound and complete w.r.t the question as well as any background information (passage, knowledge base, common sense and universal facts, etc).\\
% \textbf{Question Generation} needs the question to be related to the base material it is based upon (i.e., passage/image, etc) and additionally be answerable with the given information. Unlike the previous cases, an additional degree of freedom of creativity is unlocked in this task, due to the diversity of possible questions.\\
% \textbf{Data to Text generation:} (such as summarizing tables with sentences) It is important to preserve the facts as well as be exhaustive in verbalizing the information (verify second part).\\
% \textbf{Automated Dialogue} agents need to "listen" to the other speaker, thereby adequately respond. Be coherent with the agent's own previous utterances (consistency), as well as the other speaker's utterances. Given the diversity of possible ways a dialogue can proceed, creativity and engagingness are important for chatbot evaluation.\\
% \textbf{Image Captioning:} the caption should be relevant to the image and consistent. Although it need not describe everything in the image, and can focus on the significant details, the caption cannot contradict the image. Creativity can be enhanced through connecting additional components or abstraction, as would be the case in human generated captions. However, most existing captioning datasets stick to describing the contents of the image, which is a relatively easier setup for evaluation.\\
% Other elements: Style, Persona, Emotion?

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%12/08/2020%%%%%%%%%%%%%%%%%%%
\section{Human evaluation of NLG}
Human evaluation would be ideal to evaluate the generated hypothesis and also NLG systems as a whole. However, human evaluations are difficult to obtain on a large-scale and are expensive and time consuming. Therefore human evaluations are usually reported on a sample of the data, to show advancement in an NLG model as well as to compare the correlation with automatic metrics. In this section we provide a summary of human evaluations, particularly the procedures adopted for setting up such evaluations and the parameters evaluated for various NLG tasks. 
\subsection{Human Evaluation Setup}
Depending on the budget, availability of annotators, speed and required precision  different setups have been tried for evaluating NLG systems. The different factors to consider in such an evaluation setup are as follows:
%\MK{Now reorganise the para into the following bullet points - just move apt sentences to apt bullet points - no new sentences are needed}
\begin{itemize}
    \item \textbf{Type of annotators:} The evaluators could be experts \cite{DBLP:conf/wmt/MaBG18,DBLP:conf/wmt/MaWBG19}, crowdsourced annotators \cite{DBLP:conf/emnlp/Callison-Burch09_amt_fast_cheap,kryscinski-etal-2019-neural_summ_critic,DBLP:journals/corr/abs-1910-08684_wikibio_confidence}, or even the end-users \cite{DBLP:conf/nips/GhandehariounSJ19_selfplay,DBLP:conf/naacl/SeeRKW19} as per the requirements of the task and goal of the evaluation. For example, translation task could be evaluated by bilingual experts, to ensure any subtle nuances in source language and the target language are well accounted for. Additionally in this case, having a reference translation becomes optional rather than a necessity. On the other hand, the state of chit-chat dialogue agents could be better assessed by the end-users. More generally, for any task, real-world effectiveness needs to be assessed by the end-users of the service.  %which is still not as extensively employed by the NLG community \cite{DBLP:journals/coling/Reiter18_validity_of_bleu}. %More generally, real-world effectiveness needs to be assessed for all the tasks by the users of the service.
    \item \textbf{Scale of evaluation:} The rating on the generated text is usually obtained on a fixed scale, with each number corresponding to an indication of a specific level of quality, called the Likert scale. However, some works \cite{DBLP:conf/eacl/GattB10_tuna,DBLP:conf/acl/BelzK11_continuous_eval} have also experimented with a dynamic/movable continuous scale that can allow the evaluator to give more nuanced judgements. An alternate setting asks humans to assign a rating based on the amount of post-editing required, if any, to make the hypothesis acceptable \cite{bojar-etal-2014-findings,DBLP:journals/corr/abs-1807-02202_chaganty}. The evaluators could also be asked for binary judgements rather than a rating to indicate whether a particular criteria is satisfied or not. This binary scale is sometimes preferred over a rating scale, which usually contains 5 or 7 points, in order to force judges to make a clear decision rather than give an average rating (i.e., the middle score) \cite{horbach-etal-2020-linguistic_approp}. By extension, any even-point rating scale could be used to avoid such indecisiveness.
    %the sentence about post editing will also go here. Also need to mention about assigning multiple scores (one for fluency, once for adequacy, etc) %\MK{talk about using even numbered scales which do not allow for sitting on the fence v/s using an odd numbered scale which has a neutral rating}. 
    \item \textbf{Availability of reference and context:} To evaluate a generated text for a given NLG task, the human evaluators are usually provided with a reference and/or the context of the task, along with the text to be evaluated. Evaluation of fluency is usually performed directly on the generated text, without using the reference. References are helpful when the evaluation criteria can be reduced to a problem of comparing the similarity of information contained in the two texts. For example, a generated translation can be evaluated for soundness (coherence) and completeness (adequacy) by checking with the information in the reference. However, for most of the NLG tasks the  contexts contain more thorough information that simply cannot be captured by a set of references. Therefore contexts are necessary to evaluate the overall correctness of the generated texts. %for Dialogue,   %the reference would only be one of the many possible  %Contexts, are provided wherever it is relevant in judging a particular criteria for task fulfillment. %(Give example here). %richer supplement for evaluation.
    \item \textbf{Absolute v/s relative evaluation :} The hypothesis could be evaluated individually or by comparing it with other hypotheses. In an individual hypothesis evaluation, the candidate is provided an absolute rating for each criteria. The comparison setup could either ask to compare the ratings of the hypotheses \cite{DBLP:conf/emnlp/NovikovaDCR17} or ask for a preference order on the multiple hypotheses presented \cite{DBLP:conf/cvpr/VedantamZP15_CIDEr,DBLP:conf/eacl/KilickayaEIE17_wmd_ic,DBLP:journals/csl/DusekNR20_e2enlg}.%, usually allowing ties \cite{DBLP:journals/csl/DusekNR20_e2enlg}.
    This could also be just be a pairwise comparison \cite{DBLP:journals/corr/abs-1909-03087_acute_eval,li2017adversarial,DBLP:conf/acl/DhingraFPCDC19_parent}. Under relative ranking setup, ties are permitted and different NLG systems are compared based on the number of times they were preferred (wins), losses and ties.
    %Talk about ranking and (wins, ties, losses)
    \item \textbf{Providing Rationale :} The evaluators might additionally be asked to provide reasons for their decisions, by highlighting the corresponding text, \cite{DBLP:journals/corr/abs-1807-02202_chaganty} (any other methods?). (still todo)
    %\item Did I miss anything 
\end{itemize}
%The human evaluators could be experts or even new to the task.
%To evaluate a generated text for a given NLG task, the human evaluators are usually provided with a reference and/or the context of the task, along with the text to be evaluated.  %supplemented with the 
%The sentences to be evaluated are presented to  
%The human annotators might be asked to score the hypothesis individually or compare it against another hypothesis. %The context or background information is usually provided for getting more informed evaluations, although some studies skip this information.\\
%The score is usually obtained on a fixed scale, with each number corresponding an indication of a specific level of quality, called the Likert scale \MK{talk about using even numbered scales which do not allow for sitting on the fence v/s using an odd numbered scale which has a neutral rating}. However, some works \cite{DBLP:conf/eacl/GattB10_tuna,DBLP:conf/acl/BelzK11_continuous_eval} have also experimented with a dynamic/movable continuous scale that can allow the evaluator to give more nuanced judgements. %be finetuned to each evaluator. 
%Another setup asks for a preference order on the multiple hypotheses presented, usually allowing ties \cite{DBLP:journals/csl/DusekNR20_e2enlg}. This could also be just be a pairwise comparison \cite{DBLP:journals/corr/abs-1909-03087_acute_eval,li2017adversarial,DBLP:conf/acl/DhingraFPCDC19_parent}. %an indication of which of the multiple hypotheses presented is better than the others, usually allowing ties. 
%\cite{DBLP:journals/corr/abs-1807-02202_chaganty} explores the 
%An alternate setting asks humans to assign a rating based on the amount of post-editing required, if any, to make the hypothesis acceptable \cite{bojar-etal-2014-findings,DBLP:journals/corr/abs-1807-02202_chaganty}. \\ %number of post-edits made on the hypothesis to make it appropriate.\\
Irrespective of the setup being used, it is important to have sufficient inter-annotator agreement, which is usually measured using Cohen's Kappa or Fleiss Kappa co-efficient or Krippendorff’s alpha. %\MK{aren't there other measures - Jaccard similarity? simple precision/recall between annotators}. %Need to list down other terms and measures here. %Less popularly,
Alternatively, although not popularly, IAA could be measured using Jaccard similarity, or an F1-measure (based on precision and recall) \cite{bosch_2020}. %BLEU-Neighbours uses spearman correlation of human annotators

Achieving a high-enough inter-annotator agreement is more difficult on some of the NLG tasks which have room for subjectivity \cite{amidei-etal-2018-rethinking_agreement_iaa}. Discrepancy in IAA can occur due to (i) human-error (ii) inadequacy of the guidelines or setup (iii) ambiguity in the text \cite{DBLP:journals/nle/SampsonB08}.  %than the others. %or different assumptions
\citet{DBLP:journals/corr/abs-1807-02202_chaganty} find that asking the evaluators to highlight the portion of the text that lead to their decision or rating helps in getting better agreement. Alternatively, \citet{DBLP:conf/emnlp/NemaK18_qbleu} arrange for a discussion between the annotators after the first round of evaluation, so as to mutually agree upon the criteria for the ratings.
%Likert scale: (getting a score on a scale, say 1-5).
%Also check \citet{DBLP:conf/emnlp/NovikovaDCR17} for comments on human scale varying from metric scale, and that extremes are easily classified than middle scores. "While discrete, ordinal scales are the dominant method, a continuous scale - for example, one involving a visually presented slider (Gatt \& Belz, 2010; Belz \& Kow, 2011) - might give subjects the possibility of giving more nuanced judgements." \\
%Acute-EVAL by \citet{DBLP:journals/corr/abs-1909-03087_acute_eval} : Humans compare models and pass pairwise judgement based on preference. Pitched in the context of dialogues.\\
%Post edit rating; highlight the text regions that support the human decisions. %Collecting feedback from end users, (teachers for poilcy learning (Chang et.al 2017) - ignore for now), experts or crowd-sourced.

%\MK{Say that the humans also need to be provided with clear guidelines and these differ from task to task as explained in the next sub-section}
The human evaluators need to be provided with clear and sufficient guidelines in order to get reliable judgements. The outline of these guidelines varies across the different NLG tasks, as explained in the next subsection.
\subsection{Evaluating the Fulfillment of Task Requirements}
Most human evaluations are based on checking for task fulfillment as a whole. That is, humans are asked to rate or compare the generated sentences (and the generating systems) to indicate how satisfactorily it meets the task requirements overall. However, evaluations can also be performed at a more fine-grained level where the various contributing factors are individually evaluated. %This could also be modelled as  \cite{DBLP:conf/acl/LoweNSABP17ADEM,DBLP:conf/wmt/MaBG18,DBLP:conf/wmt/MaWBG19,ghazarian19}.\\ %Ghazarian -> not appropriate to very appropriate. ADEM- overall quality of the response. RUBER -> human satisfaction of a reply.
%These factors/criteria vary in number, meaning and amount of applicability for each task. We hence discuss the set of criteria for each task separately, except for `Fluency' which is common across all the NLG tasks.
One such factor to be considered for evaluating the generated texts is `fluency'.
\begin{itemize}
    \item \textbf{Fluency} refers to correctness of the generated text with respect to grammar and word choice, including spellings. %/syntactical
\end{itemize}
% \begin{table}[h]
%     \centering
%     \begin{tabular}{|c|c|c|c|c|}
%     \hline
%          \multicolumn{5}{|c|}{How do you judge the fluency of the candidate sentence?} \\
%          \hline
%          1. Incomprehensible & 2. Not fluent German & 3. Non-native German & 4. Good German & 5. Flawless German\\
%          \hline
%     \end{tabular}
%     \caption{An example question used for evaluating fluency \cite{callison-burch-etal-2006-evaluating_bleu_in_mt}}
%     \label{tab:fluency_example}
% \end{table}
%For example, Table \ref{tab:fluency_example} shows a sample 5-point Likert scale used for the evaluation of Fluency \cite{callison-burch-etal-2006-evaluating_bleu_in_mt}.
%a question, ``How do you judge the fluency of this sentence?" could be followed by a 5-point rating scale: \\
%1. Incomprehensible 2. Not fluent German 3. Non-native German 4. Good German 5. Flawless German \cite{callison-burch-etal-2006-evaluating_bleu_in_mt}.
To evaluate this, evaluators might be asked a question such as, ``How do you judge the fluency of this text?" followed by a 5-point rating scale \cite{callison-burch-etal-2006-evaluating_bleu_in_mt}: \\
1. Incomprehensible 2. Not fluent German 3. Non-native German 4. Good German 5. Flawless German\\
Instead of a 5-point scale, other scales with different quality ratings could be used: ``How natural is the English of the given sentence?'' 1. Very unnatural 2. Mostly unnatural 3. Mostly natural 4. Very natural \cite{DBLP:conf/naacl/SeeRKW19}. 
Another possibility is to present multiple candidate sentences and ask the evaluator, ``Which of these sentences seems more fluent?". The evaluator then indicates a preference or a tie. %Since such questions asking for a preference que

Fluency is a relevant criteria for all the tasks. However, the list of factors/criteria used for evaluation varies in number, meaning of the factors and amount of significance/applicability for each task. We hence discuss the set of criteria for each task separately now, leaving out fluency.
%We now discuss the criteria for all the tasks individually.
\\
\textbf{Machine Translation:} Bilingual experts are presented with the source sentence and the hypothesis. Alternatively, monolingual annotators can be presented with the reference sentence and the hypothesis to judge (i) Fluency and (ii) Adequacy of the hypothesis \cite{DBLP:journals/nle/GrahamBMZ17_crowd_alone}. 
\begin{itemize}
    %\item \textbf{Fluency} refers to grammatical/syntactical correctness of the generated text
    \item \textbf{Adequacy} is to check if the hypothesis adequately represents all the information present in the reference. To quantify this measure, an example setup used \cite{callison-burch-etal-2006-evaluating_bleu_in_mt} is How much of the meaning expressed in the reference translation is also expressed in the hypothesis translation? 1. None 2. Little 3. Much 4. Most 5. All
\end{itemize}
% For example, annotators might be presented with the following question to measure adequacy
% \begin{table}[h]
%     \centering
%     \begin{tabular}{|x{2.3cm}|x{2.3cm}|x{2.3cm}|x{2.3cm}|x{2.3cm}|}
%     \hline
%          \multicolumn{5}{|c|}{How much of the meaning expressed in the reference translation is also expressed in the hypothesis translation? } \\
%          \hline
%          1. None & 2. Little & 3. Much & 4. Most & 5. All \tn
%          \hline
%     \end{tabular}
%     %\caption{An example question used for evaluating adequacy \cite{callison-burch-etal-2006-evaluating_bleu_in_mt}}
%     \label{tab:adequacy_example}
% \end{table}
%Example: How much of the meaning expressed in the reference translation is also expressed in the hypothesis translation? 
%1. None 2. Little 3. Much 4. Most 5. All \cite{callison-burch-etal-2006-evaluating_bleu_in_mt}
%`Fluency' refers to the grammatical/syntactical correctness of the generated text. `Adequacy' parameter is to check if the hypothesis adequately represents the information present in the reference.
%To check if the generation translation is correct, bilingual experts are presented with the source sentence and the hypothesis. \citet{DBLP:journals/nle/GrahamBMZ17_crowd_alone} alternatively propose having monolingual evaluators to verify for two parameters: (i) Fluency and (ii) Adequacy individually. Fluency can be determined directly on a generated text. However, measurement of adequacy needs a reference translation and is modelled as checking if the hypothesis adequately represents the information present in the reference. \MK{Need to define fluency and adequacy with examples}\\ 
\textbf{Abstractive Summarization:} Human evaluators are presented with either the document to be summarized or a set of references along with the candidate summary. The parameters usually used for evaluation include informativeness and coherence \cite{DBLP:conf/ntcir/Mani01,mani-etal-1999-improving}. %considered valuable
Instead of coherence, the text quality could be sub-divided into grammaticality, non-redundancy, referential clarity, structure and coherence \cite{DBLP:journals/cai/SteinbergerJ09,DBLP:journals/lre/LloretPA18}. Therefore the relevant factors include:
\begin{itemize}
    \item \textbf{Informativeness:} The summary should convey the key points of the text. 
    For instance, a summary of a biography should contain the significant events of a person's life. We do not want a summary that only quotes the person's profession, nor do we want a summary that is unnecessarily long/verbose.
%     \item \textbf{Coherence:} The summary needs to be consistent with the information present in the document.
%     Example: 
% \end{itemize}
% Additionally, a candidate summary should also be assessed for the following \cite{DBLP:journals/cai/SteinbergerJ09,DBLP:journals/lre/LloretPA18}:
% \begin{itemize}
    %\item Grammaticality: Correct grammar
    \item \textbf{Non-redundancy:} The summary should not repeat any points, and ideally have maximal information coverage within the limited text length.
    \item \textbf{Referential clarity:} Any references in the summary should be unambiguous and within the scope of the summary. Any nouns, pronouns or specific information must be referred to clearly in the summary. 
    \item \textbf{Focus:} The summary needs have a focus and all the sentences need to contain information related to the summary.
    \item \textbf{Structure and Coherence:} The summary should be a well-organized and coherent body of information, not just a heap of related information. Specifically, the sentences should be connected to one another maintaining good information flow.
    % \begin{table}[h]
    %     \centering
    %     \begin{tabular}{|p{6.5cm}|p{6.5cm}|}
    %     \hline
    %          \multicolumn{2}{|c|}{Which summary has better structure and coherence?} \\
    %          \hline
    %         Terry’s career as a photographer came after he failed to make it as a punk rock musician. He got  his  first  big  break  in  1994  with a shoot for Vibe magazine...  & Terry’s career as a photographer came after he failed to make it as a punk rock musician. The photographer  has  also  directed  music videos in his time as a musician...\\
    %         \hline
    %     \end{tabular}
    %     %\caption{Caption}
    %     \label{tab:struct_coherence_table}
    % \end{table}
\end{itemize}
    % \begin{table}[h]
    %     \centering
    %     \begin{tabular}{|p{6.5cm}|p{6.5cm}|}
    %     \hline
    %          \multicolumn{2}{|c|}{Evaluate summaries A and B according to the above criteria} \\
    %          \hline
    %         \textbf{A:} These days we are increasingly using outdoor space for the occasional barbecue or to relax in a hot tub rather than for tending flowers, according to researchers. As  a  result,  only  a  handful  of  traditional flowers still grow in English country gardens, with the  average  one  usually  containing  a  mere  four species- daffodils, crocuses, roses and tulips. & \textbf{B:} These days we are increasingly using outdoor space for the occasional barbecue or to relax in a hot tub rather than for tending flowers, according to researchers. Sir Roy Strong, the landscape designer of it, told the Sunday Times: `British people used to take pride in having neat gardens with lots of flowers. But now all the gardening land and time goes into barbecues and relaxing in tubs.'\\
    %         \hline
    %         \multicolumn{2}{|l|}{\textbf{Non-Redundancy:} A is preferred since both the sentences in B make the same point.} \\
    %          \hline
    %          \multicolumn{2}{|l|}{\textbf{Referential clarity:} B does not clarify what `it' refers to in ``landscape director of it".} \\
    %          \hline
    %          \multicolumn{2}{|l|}{\textbf{Focus:} While both A and B refer to the decline of the English gardens, A is better focused.} \\
    %          \hline
    %     \end{tabular}
    %     %\caption{Caption}
    %     \label{tab:struct_coherence_table}
    % \end{table}
%Conciseness and faithfulness (misinformation?)
%Informativeness and coherence are considered valuable dimensions for summary evaluation \cite{DBLP:conf/ntcir/Mani01,mani-etal-1999-improving}. \cite{DBLP:journals/cai/SteinbergerJ09,DBLP:journals/lre/LloretPA18} additionally discuss the parameters of grammaticality, non-redundancy, referential clarity, focus, as well as structure and coherence to be essential in a good summary. \MK{Need to define informativeness, coherence, \textit{etc.} with examples} \\ 
% considers the 2 major % use an expanded set of human evaluation parameters to include 
%The human evaluators can check for the correct identification of the key idea or the few main points which are to be summarized, along with fluency and coherence of the summary with the original text.\\
\textbf{Question Answering:} Human evaluators are sometimes first presented with the question and answer to check if the answer is plausible \cite{DBLP:journals/corr/abs-1807-02202_chaganty}. When the context passage/image is provided, the aim is to check whether the answer is correct and consistent with the context. Alternatively, since question answering datasets are usually provided with gold standard answers for each question, the judges might simple be asked how closely the candidate answer captures the same information as the gold standard answer.
\\
%The task where the answers are to be generated (instead of selected from the text or out of given options) need to be checked for adequately addressing the question and maintaining coherence with the question as well as any background information (passage, knowledge base, common sense and universal facts, etc). \citet{DBLP:journals/corr/abs-1807-02202_chaganty} ask human annotators to first judge whether the answer is plausible for the question and then present the context to identify whether the answer is correct. \\
\textbf{Question Generation:} The candidate questions are presented to the evaluators usually along with the context (passage/image, etc, on which the questions are needed). This may be accompanied with a set of candidate answers \cite{DBLP:conf/naacl/Hosking019} although they are usually not provided, even if available in the dataset, to avoid any bias in the free-form question generation task \cite{DBLP:conf/emnlp/NemaK18_qbleu}.
The factors considered to judge the generated questions include \cite{DBLP:conf/emnlp/NemaK18_qbleu,DBLP:conf/naacl/Hosking019}:
\begin{itemize}
    %\item Fluency:
    \item \textbf{Relevance}: The questions need to be related to the material they are based upon. 
    \item \textbf{Answerability}: The generated question should be answerable given the context. A question might be deemed unanswerable due to its lack of completeness or sensibility, or even if the information required to answer the question is not found in the context. The last case could be acceptable to some extent since such questions can be answered stating the insufficiency of information, however having too many questions of such form is futile for the task. %, answerability is desired and important for generating meaningful questions overall. 
    \end{itemize}
%As \citet{DBLP:conf/emnlp/NemaK18_qbleu} point out, `Answerability' is an important criteria to evaluate the generated questions. This is in addition to the other contributing factors such as fluency, and relevance (or faithfulness) to the base material, i.e., passage/image, etc, on which the questions are based \cite{DBLP:conf/naacl/Hosking019}. \cite{DBLP:conf/emnlp/NemaK18_qbleu} discuss the two ways of presenting the candidate questions to humans, viz., either the standalone questions or the questions along with the base material. \MK{Need to define all the metrics that we have}\\
\textbf{Data to Text generation:} %It is important for the text to preserve the facts as well as be adequate in verbalizing the information present in the data. 
Human judges are shown the text along with the data (i.e., table, graph, etc). The factors considered for human evaluation vary slightly in different works such as WebNLG challenge \cite{shimorina2019webnlg_human_eval}, E2E NLG dataset \cite{DBLP:journals/csl/DusekNR20_e2enlg} or WikiBio dataset \cite{DBLP:journals/corr/abs-1910-08684_wikibio_confidence}. %\cite{shimorina2019webnlg_human_eval,DBLP:journals/csl/DusekNR20_e2enlg,DBLP:journals/corr/abs-1910-08684_wikibio_confidence,DBLP:conf/acl/DhingraFPCDC19_parent}. 
Here, we discuss the more fine-grained sub-division of `semantic adequacy' parameter used in \cite{shimorina2019webnlg_human_eval} into faithfulness and coverage as done in \cite{DBLP:journals/corr/abs-1910-08684_wikibio_confidence,DBLP:conf/acl/DhingraFPCDC19_parent}.
\begin{itemize}
    \item \textbf{Faithfulness:} It is important for the text to preserve the facts. For example, any text that misrepresents the year of birth of a person would be unacceptable and would also be ranked lower than a text that does not mention the year at all.
    \item \textbf{Informativeness or Coverage:} The text needs to adequately verbalize the information present in the data. As per the task requirements, coverage of all the details or the most significant details might be desired.
\end{itemize}
%The WebNLG challenge procures human judgements on 3 criteria: Fluency (or naturalness), Grammar and Semantic adequacy (i.e., correctly representing the meaning in the data) \cite{shimorina2019webnlg_human_eval}. On E2E NLG dataset, \cite{DBLP:journals/csl/DusekNR20_e2enlg} instead obtain human rankings on the candidates by evaluating naturalness and quality in separate crowdsourcing tasks, where for fluency, the text is not accompanied by the input data, unlike in the setup for ranking overall quality. \cite{DBLP:conf/acl/DhingraFPCDC19_parent} obtain pairwise preference in terms of Naturalness, Faithfulness, and Informativeness on WikiBio. \\ %Also on WikiBio, \cite{DBLP:journals/corr/abs-1910-08684_wikibio_confidence} fluency, faithfulness and coverage, but not on pairwise.
\textbf{Automated Dialogue} %agents need to "listen" to the other speaker, thereby adequately respond. That is, the generated response should be coherent with the agent's own previous utterances, as well as the other speaker's utterances. 
Dialogue generation task has relatively more parameters to be considered while comparing or evaluating dialogue responses and systems. One way to categorize these parameters, adopted by \cite{DBLP:conf/naacl/SeeRKW19}, is presented below along with the corresponding questions provided to the human evaluators to evaluate each of these:
\begin{itemize}
    %\item Fluency
    \item \textbf{Making sense:} Does the bot say things that don't make sense?
    \item \textbf{Engagingness:} Is the dialogue agent enjoyable to talk to?
    \item \textbf{Interestingness:} Did you find the bot interesting to talk to?
    \item \textbf{Inquisitivenes:} Does the bot ask a good amount of questions?
    \item \textbf{Listening:} Does the bot pay attention to what you say?
    \item \textbf{Avoiding Repetition:} Does the bot repeat itself? (either within or across utterances)
    \item \textbf{Humanness:} Is the conversation with a person or a bot?
\end{itemize}
Often for dialogue evaluation, instead of separately evaluating all these factors, the evaluators are asked to simply rate the overall quality of the response \cite{DBLP:conf/acl/LoweNSABP17ADEM,DBLP:conf/aaai/TaoMZY18ruber}, or specifically asked to check for relevance of the response \cite{ghazarian19}. For task-oriented dialogues, additional constraints are taken into consideration, such as providing the appropriate information or service, guiding the conversation towards a desired end-goal, etc. In open-domain dialogue settings also, additional constraints such as persona adherence \cite{personachat}, emotion-consistency \cite{DBLP:conf/nips/GhandehariounSJ19_selfplay}, etc, are being used to expand the domain boundaries and challenge the state-of-the-art.
%\cite{DBLP:conf/naacl/SeeRKW19} evaluate conversation systems for  Engagingness, Interestingness, Inquisitiveness, Listening, Avoiding Repetition, Fluency, Making Sense, Ease of Persona retrieval, apart from Humanness. \cite{DBLP:conf/acl/LoweNSABP17ADEM} simplify this by asking evaluators to score the overall quality of the response.  Often evaluators are asked to specifically check relevance of the response \cite{ghazarian19}, or human satisfaction \cite{DBLP:conf/aaai/TaoMZY18ruber}. For task-oriented dialogues, additional constraints are taken into consideration, such as providing the appropriate information or service, guiding the conversation towards a desired end-goal, etc. \MK{All these confusing parameters need to be defined and explained with examples}\\ %steering
\\
\textbf{Image Captioning:} The caption should be relevant to the image and adequately explain the image. This criteria is checked by asking annotators to evaluate `Relevance' and `Thoroughness' of the caption by presenting it along with the corresponding image \cite{DBLP:journals/cviu/AdityaYBAF18_image_understanding}.
\begin{itemize}
    \item Relevance: This measures how well the caption is connected to the contents of the image. 
    \item Thoroughness: The caption needs to adequately describe the image. Usually the task does not require a complete description of everything in the image and caption can mostly focus on the main subjects/actions in the image and any significant details.
\end{itemize}%\cite{DBLP:conf/eccv/SharifWBS18_nneval} obtain caption relevance scores from the annotators. %Although it need not describe everything in the image and can mostly focus on the significant details, the caption cannot contradict the image.
%\subsubsection{Human-likeness:} Often the human evaluation for these various tasks is summarized into one entity measuring how human-like the generated sentence is.
%\subsection{Evaluating Contributing Factors Individually}
%Evaluations can also be performed at a more fine-grained level where different factors are individually scored. % as done by \citet{DBLP:journals/corr/abs-2005-00583_maude,DBLP:conf/naacl/SeeRKW19}.\\
%The factorization is task-specific and the level of granularity varies. %\cite{DBLP:conf/naacl/SeeRKW19} and \cite{DBLP:journals/corr/abs-2005-00583_maude} evaluate conversation systems for for Engagingness, Interestingness, Inquisitiveness, Listening, Avoiding Repetition, Fluency, Making Sense, Ease of Persona retrieval, and Humanness. %\cite{DBLP:conf/emnlp/NemaK18_qbleu} evaluate the task of Question Generation using the parameter of `answerability'.
\MK{Regarding Section 2 and 3: I feel that section 2 should just be at an introductory/intuitive level without formally defining these metrics. Section 3.2 is where we should formally define all the metrics. Each para in section 32. should have the following format: <Task Name>: Human evaluators are shown xyz and asked to judge the generated response based on the following criteria - Bulleted list of criteria with definition/example/explanation of each. Overall, sections 2 and 3 are the most important - simply because they appear early on in the paper and we need to make a good early impression. Having said that, both sections are developing well and in one more iteration we will get very close to what we want. }


==> xmet.tex <==
METEOR universal: universal parameter set is "learned from pooling human judgments of translation quality from several language directions."

Word based
Often these are deconstructed to the constituent words to facilitate better comparison of sentences or paragraphs. That is, the words can be compared rather than matching the strings. These metrics operate at the word-level, by checking for word overlap, or overlap of n-contiguous-words called n-grams, between the hypothesis and the reference, or even counting the number of edits required to make the hypothesis similar to the reference.
Since words are functional units of a sentence, each with an associated meaning
